Stability of superthermal strahl electrons in the solar wind

We present a kinetic stability analysis of the solar wind electron distribution function consisting of the Maxwellian core and the magnetic-field aligned strahl, a superthermal electron beam propagating away from the sun. We use an electron strahl distribution function obtained as a solution of a weakly collisional drift-kinetic equation, representative of a strahl affected by Coulomb collisions but unadulterated by possible broadening from turbulence. This distribution function is essentially non-Maxwellian and varies with the heliospheric distance. The stability analysis is performed with the Vlasov-Maxwell linear solver LEOPARD. We find that depending on the heliospheric distance, the core-strahl electron distribution becomes unstable with respect to sunward-propagating kinetic-Alfv\'en, magnetosonic, and whistler modes, in a broad range of propagation angles. The wavenumbers of the unstable modes are close to the ion inertial scales, and the radial distances at which the instabilities first appear are on the order of 1 AU. However, we have not detected any instabilities driven by resonant wave interactions with the superthermal strahl electrons. Instead, the observed instabilities are triggered by a relative drift between the electron and ion cores necessary to maintain zero electric current in the solar wind frame (ion frame). Contrary to strahl distributions modeled by shifted Maxwellians, the electron strahl obtained as a solution of the kinetic equation is stable. Our results are consistent with the previous studies based on a more restricted solution for the electron strahl.

==> include/defs.tex <==

% Counter for keeping track of comments
\newcounter{revcomcounter}

% Command for reading the review comment counter
\renewcommand{\therevcomcounter}{\arabic{revcomcounter}}

% Review comment environment
\newenvironment{revcom}[1][]{%
\refstepcounter{revcomcounter}%
\ifx\\#1\\%
\else
\label{#1}%
\fi
\begin{trivlist}\item\textbf{Comment~\therevcomcounter: }\em%
}%
{\end{trivlist}}%

% Environment for responding to review comments
\newenvironment{response}[1][]{%
\begin{trivlist}\item\textbf{Response: }%
}%
{\end{trivlist}}%

